Accelerating Multilingual Language Model for Excessively Tokenized Languages

Recent advancements in large language models (LLMs) have remarkably enhanced performances on a variety of tasks in multiple languages. However, tokenizers in LLMs trained primarily on English-centric corpora often overly fragment a text into character or Unicode-level tokens in non-Roman alphabetic languages, leading to inefficient text generation. We introduce a simple yet effective framework to accelerate text generation in such languages. Our approach involves employing a new language model head with a vocabulary set tailored to a specific target language for a pre-trained LLM. This is followed by fine-tuning the new head while incorporating a verification step to ensure the model's performance is preserved. We show that this targeted fine-tuning, while freezing other model parameters, effectively reduces token fragmentation for the target language. Our extensive experiments demonstrate that the proposed framework increases the generation speed by a factor of 1.7 while maintaining the performance of pre-trained multilingual models on target monolingual tasks.

==> Sections/02-background.tex <==

% TODO: Tokenization -> Text Generation

% Tokenization
% n-gram level sequences. 
% n-gram level sequences. 


% TODO: Background -> (Preliminary Study) 에 대한 및 자문 구하기? (교수님?, 태희형?) -> 문제의식을 명확히 보여줄만한 실험.

% Case Study 자체에서는 finely tokenizatioon에만 집중하는게 어떨까?****************234ㄱ5 

% 문제의식을 보여줄수 있는 실험 하나더 추가!! 
% ahia-> few-shot prompting조차 불가
% text generation speed를 확연하게 보여줄수 있는 실험이 선행되어야 할거 같음
% decoding step을 비교해야할까? -> too trivial
% latency per sample~ -> 언어별로 보여주는게 클리어할것 같음. llama-multilingual model 기반으로 inference 해보기.

% latency per sample~ -> 언어별로 보여주는 것이 클리어할것 같음. multilingual llama model 기반으로 inference 해보기 korean / japanese -> 
% 생성해야할 토큰의 개수가 큰 테스크별로 확장해서 measure해보기. 

% \subsection{Over-Tokenization on Monolingual Scripts}
% \input{Sections/table/overly_tokenization}

% A simple examination of "over tokenization" can be conducted by contrasting the tokenization results between multilingual and monolingual tokenizers.
% We choose 3 representative language model that is trained including multilingual corpora, or broadly utilized service across nations.
% For the monolingual scripts, we use FLoRes-200 which is composed  Wikipedia articles and covering
% a variety of different topics and domains with translated sentence into 200 languages.
% Table~\ref{tab:flores} shows the average number of resulting tokens for 3 languages. In overall, english-centric model excessively tokenize on Japanese and Korean Scripts, comparing with English scripts. 
% The issue of "over-tokenization" can be thoroughly examined by comparing the tokenization results between multilingual and monolingual tokenizers. 
% We selected three representative language models Bloomz, Llama-2, GPT-4 that have been trained on multilingual corpora or are widely used across various nations. 
% For the monolingual scripts, we utilized the FLoRes-200 dataset, which comprises Wikipedia articles covering a diverse range of topics and domains, translated into 200 languages.
% As shown as the Table~\ref{tab:flores}, all of multilingual tokenizer produce more token comparing with monolingual tokenizer.
% \input{Sections/table/overly_tokenization}

% \paragraph{Language Modeling} 
% % The objective of auto-regressive language modeling is to establish a probability distribution $p_{\theta}(\mathbf{x})$, where $\theta$ is the parameter of model, over a sequence of tokens $\mathbf{x} = [x_1,\ldots, x_T]$ from a pre-defined vocabulary $\mathcal{V}$, where $x_t \in \mathcal{V}$.
% The goal of auto-regressive language modeling is to create a probability distribution, denoted as $p_{\theta}(\mathbf{x})$, where $\theta$ represents the model parameter. This distribution is established over a sequence of tokens, represented as $\mathbf{x} = [x_1,\ldots, x_T]$. These tokens are derived from a pre-established vocabulary, denoted as $\mathcal{V}$, where each token $x_t$ is a member of $\mathcal{V}$.
% A conventional approach involves maximizing the log-likelihood of a sequence: 
% \begin{equation}\label{eq:log-likelihood}
% \max_{\theta}\mathcal{L}_{\text{MLE}}(p_{\theta}, \mathbf{x}) = \sum_{t=1}^{T}\log p_{\theta}(x_t|\mathbf{x}_{<t}).    
% \end{equation}

% \begin{equation} 
% p_{\theta}(x_t|\mathbf{x}_{<t}) = \operatorname{Softmax}(f_{\theta}^{o}(\mathbf{h}_{t-1})) \in \mathbb{R}^{|\mathcal{V}|}
% \label{eq1}
% \end{equation}
% where $\mathbf{h}_{t-1} \in \mathbb{R}^{d}$ is a hidden state of the context $\mathbf{x}_{<t}$; $f_{\theta}^{o}\in \mathbb{R}^{ d\times|\mathcal{V}|}$ is a output layer of model $f_\theta$ to predict next token $x_t \in \mathcal{V}$, respectively. 
% The $f_{O}(\mathbf{h}_{t-1})$ is consisted of dot product $h_{t-1}~\cdot~W_O$ which is called a \textit{logit}.

\paragraph{Tokenization in LM}
Tokenization is the process of segmenting text into subword chunks~\citep{kudo-2018-subword,sennrich2015neural}. 
The process can be started with a base vocabulary composed solely of \textit{characters}, then, new vocabulary items are subsequently added by recursively merging existing ones based on the frequency statistics within a training corpus.
However, in a multilingual setup, even a base vocabulary composed solely of characters can be extensive, with over 130K items~\citep{wang2019neural}. 
% Moreover, character-based Byte Pair Encoding (BPE) is not exempt from out-of-vocabulary (OOV) issues on new scripts~\citep{wang2019neural}.

\paragraph{Byte-level Subword Tokenization}
\citet{radford2019language} proposed using \textit{bytes} as the basic units, with only 256 tokens required to form subwords. 
This Byte-level Byte Pair Encoding (BBPE) does not suffer from out-of-vocabulary problem and has become the standard in most pre-trained models~\citep{brown2020language,muennighoff2022crosslingual,zhang2022opt,Scao2022BLOOMA1}. 
% BBPE does not suffer OOV problem and allows for script-agnostic vocabulary construction, even enabling the support of new scripts without modifying the vocabulary. 
However, BBPE often produces longer sequence length when handling multilingual scripts compared to character-based BPE~\citep{wang2019neural,petrov2023language}. 
% Recently, \citet{ahia2023all} shows that the number of BBPE-based tokenization results across languages is not just determined by the proportion of text from language in the pretraining data but also by language/script properties.


% As depicted in the Table 1, BBPE-based tokenizers excessively segment texts into a sequence of several bytes.
% \input{Sections/table/overly_tokenization}
% The tokenization process is to convert text into subword chunks. 
% It can be started with a base vocabulary of only \textit{characters} and adds new vocabulary items by recursively merging existing ones based on their frequency statistics in a training corpus. 
% However, in the context of multilingual setup, that contain data in a variety of scripts, character-based BPE is not free from out-of-vocabulary(OOV) issues.
% Instead, recent work~\citep{radford2019language} proposed using bytes as the basic units with only 256 tokens to compose subwords.
% % using a \textit{byte-level} base vocabulary with only 256 tokens.
% The Byte-level byte pair encoding (BBPE) become the de facto standard using in most pre-trained model.
% BBPE does not produce unknown token, and makes vocabulary construction script-agnostic, even allowing new scripts to be supported later on without modifying the vocabulary. 
% % However, byte as base이 사라지는 대신에, base vocabulary의 단위가 character에 비해 더 작아진 형태이므로 전체적인 token length가 길어질 것이다.
% However, BBPE often produce longer sequence length when dealing with multilingual sources comparing with character-based BPE~\cite{wang2019neural}.
% As depicted in Table~\ref{tab:overly_tokenization}, BBPE tokenize a character into several bytes with the base vocabulary of bytes. 
% However, not only are different scripts encoded differently, their distribution in the training corpora varies widely.

% \paragraph{Exccessive Fragmentation} 
% % \jm{We aim to investigate the issue of excessive fragmentation~\citep{ ahia2023all,petrov2023language} in the multilingual setup, a problem where a tokenizer generates an excessive number of tokens when the input texts significantly differ from the statistics of the pre-trained corpus~\cite{rust-etal-2021-good, hong2021avocado}.}
% % Concretely, we compared the tokenization output of several multilingual model tokenizers: Bloomz~\citep{Scao2022BLOOMA1}, Llama-2~\cite{touvron2023llama}, and GPT-3.5/4~\citep{gpt4openai} with monolingual counterparts using the FLoRes-200~\citep{goyal2022flores} dataset.\footnote{ \url{EleutherAI/polyglot-ko-12.8b} for Korean, \url{rinna/japanese-gpt-neox-3.6b} for Japanese.} 
% % This dataset encompassing Wikipedia articles in 200 languages. 
% % The results, as depicted in the table~\ref{tab:flores}, reveal a consistent pattern: multilingual tokenizers generate a higher number of tokens compared to their monolingual counterparts for Japanese and Korean languages.
% % The issue of excessive-fragmentation is an inherent challenge in the field of multilingual tokenizers~\citep{rust-etal-2021-good,zhang2022robust,ahia2023all,petrov2023language}. 
% % This is primarily due to the impracticality of integrating more than a hundred languages into a single model while maintaining a balanced vocabulary composition for all languages~\citep{wang-etal-2019-improving}.
% % Moreover, the number of items in the vocabulary increases, the size of the model parameters expands exponentially, thereby significantly impacting training efficiency~\cite{liang2023xlm}.
% We explore the issue of excessive fragmentation~\citep{ ahia2023all,petrov2023language} in multilingual setups, a common challenge in multilingual tokenizers~\citep{rust-etal-2021-good,zhang2022robust,ahia2023all,petrov2023language}. The problem occurs when a tokenizer produces too many tokens due to significant differences between input texts and the pre-trained corpus~\citep{rust-etal-2021-good, hong2021avocado}. 

% The difficulty of integrating numerous languages into one model while balancing vocabulary composition contributes to this issue~\citep{wang2019improving}. As the number of vocabulary items increases, model parameters expand exponentially, impacting training efficiency~\citep{liang2023xlm}. 

% To investigate this, we compared the tokenization outputs of several multilingual model tokenizers: Bloomz~\citep{Scao2022BLOOMA1}, Llama-2~\citep{touvron2023llama}, and GPT-3.5/4~\citep{gpt4openai}. We used the FLoRes-200~\citep{goyal2022flores} dataset, which includes Wikipedia articles in 200 languages. Table~\ref{tab:flores} indicates that multilingual tokenizers generate more tokens for Japanese and Korean languages than their monolingual counterparts.

% In summary, excessive tokenization on multilingual scripts becomes a significant issue due to the autoregressive nature of language model, implying the need for more efficient text generation procedures, which our study aims to address.
% This implies the need for more efficient text generation procedures, which our study aims to address.

% \subsection{Over-Tokenization Impacts Generation Speed}
% \input{Sections/table/overly_tokenization}
% \begin{figure}[t]
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=.95\linewidth]{Sections/figures/output.png}
% \end{subfigure}
% \caption{We track inference speed depending on task: one A100 GPU and bfloat16 precision.}
% % 표로 바꾸기
% \label{fig:speed_task}
% \end{figure}

% Prior work have concentrated on assessing the overall performance of multilingual language models through tasks. 
% This section aims to quantify the impact of excessive fragmentation on generation speed across various languages, thereby highlighting a significant challenge in the field of text generation. 
% We have designed tasks based on the required number of tokens for generation. 
% For instance, extractive question answering requires the generation of a limited number of n-gram words, while the summarization task necessitates the production of short sentences.
% For these experiments, we employ \textbf{TyDiQA-GoldP}~\citep{clark2020tydi} for the extractive QA task and \textbf{XLSum}~\citep{hasan2021xl} for Summarization. 
% Additionally, we have selected samples from the story writing category within the MT-Bench~\cite{zheng2023judging} and used samples translated into Korean and Japanese for further analysis.

% TODO: contribution point 요약



% As depicted in the Table~\ref{fig:speed_task}, a comparative analysis using TyDiQA shows that the generation speed remains relatively stable when dealing with single or n-gram words. 
% However, a significant difference in generation speed becomes evident when the task requires the creation of sentences that extend beyond a single sentence, as in the summarization task. 
% When comparing Summarization and MT-Bench tasks, we find that a Summarization task may have a longer prefix but requires the generation of fewer sentences. 
% Conversely, MT-Bench tasks may have a shorter prefix but require the generation of more sentences. 
% In these cases, excessive tokenization becomes a significant issue, exacerbating the challenges associated with the volume of information that the models must generate. 
% This implies the need for more efficient text generation procedures, which our study aims to address.

% As depicted in Figure~\ref{fig:speed_task}, a comparative analysis in TyDiQA reveals that the generation speed does not significantly fluctuate when handling a single or n-gram words. 
% However, a noticeable discrepancy in generation speed becomes apparent when the task necessitates the formulation of sentences that extend beyond a single sentence in summarization task.
% In the comparison between Summarization and MT-Bench tasks, we encounter instances where a Summarization task may encompass an extended prefix yet only requires the generation of a relatively fewer number of sentences. 
% On the other hand, MT-Bench tasks may feature a succinct prefix but demand the generation of a relatively larger quantity of sentences. 
% In these scenarios, excessive tokenization becomes particularly detrimental, intensifying the challenges associated with the volumn of information that the models must generate.
% In the course of our detailed examination, we endeavored to investigate the patterns exhibited by monolingual words when processed through the perspective of a multilingual model. 
% We defined the first element of a monolingual word as the 'start token' and the subsequent elements as 'continuation tokens'. 
% Take, for example, the Korean term "서울", which refers to the capital city of South Korea; it is segmented by the multilingual tokenizer into the sequence ('서', '<0xEC>', '<0xB8>', '<0x9A>'). 
% Within this N-gram, the leading "서" is designated as the start token, and the remaining sequence ('<0xEC>', '<0xB8>', '<0x9A>') is categorized as continuation tokens. 
% Following this delineation, we analyzed the propensities of these tokens by quantifying their likelihoods using the multilingual model. 
% As depicted in Figure~\ref{fig:prob_plot}, while the prediction of the start token is characterized by a degree of uncertainty, the prediction of the subsequent tokens is comparatively more deterministic.

% In our subsequent analysis, we sought to explore the tendencies of monolingual words as rendered within a writing script from the perspective of a multilingual model. 
% We designated the initial part of a monilingual word as the 'start token' and the succeeding words as 'continuation tokens'. Thereafter, we observed the tendencies of these categorized tokens by measuring their probabilities through multilingual model. 
% For instance, the term "서울", which denotes the capital of South Korea, is preprocessed by the multilingual tokenizer into ('서', '<0xEC>', '<0xB8>', '<0x9A>'). 
% Of this N-gram, the initial "서" is classified as the start token, while the ensuing sequence ('<0xEC>', '<0xB8>', '<0x9A>') is identified as continuation tokens. 
% As illustrated by the figure~\ref{fig:prob_plot} while the prediction of the token at the 'start' position is relatively uncertain, the subsequent continuation tokens are much easier to predict.

% In the section, we investigate 

% 

% \input{Sections/table/overly_tokenization}
% \begin{figure}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=.95\linewidth]{Sections/figures/output.png}
% \end{subfigure}
% \caption{Comparing the probability in start and continuation tokens in monolingual word with  multilingual model.
% }
% \label{fig:prob_plot}
% \vspace{-0.3cm}
% \end{figure}


==> Sections/05-results.tex <==
% TODO: 
% results 금방 쓰니까 실험 parallel 하게 진행해버리기.
% \input{Sections/table/main_table}
% We assessed the performance of MuMo framework against \textbf{AR} and \textbf{Spec.} across summarization, translation, and MT-bench tasks in Korean and Japanese. 

% We assessed MuMo with two types of approach: Accelerating LLM at inference and multilingual adaptation. 
% The first experiment 
% Both involve choosing the corresponding label given a finite label set for each test sample; 

% \subsection{Baselines}
% We establish several baselines for comparison. 
% The first baseline is the conventional auto0regressive language model
\textbf{(AR)}, which sequentially samples the subsequent word based on the probability distribution over the pre-trained vocabulary. 
% This approach serves as the standard against which improvements are measured.

% We also consider Speculative Sampling~\citep{chen2023accelerating,leviathan2023fast}.
% This technique utilizes a preliminary "draft" model to rapidly generate a set of token candidates at each decoding step. 
% Subsequently, these candidates undergo a validation process by the original, comprehensive language model to ascertain their likelihood as plausible continuations of the text. 
% We implement two variants of this method: one with the capability to reject unsuitable candidates \textbf{(Spec.)} and another without this rejection feature \textbf{(Spec. w/o Reject)}.
% For the draft model, we employ Llama-2-7B, which has been fine-tuned on language-specific instruction datasets.

% Lastly, we incorporate Lexical Shortlisting \textbf{(Shortlisting)}~\citep{abdaoui2020load,ushio2023efficient}. 
% This technique streamlines the decoding process by precluding tokens that are irrelevant to the target monolingual language. 
% Our implementation involves filtering out tokens that are not present within the corresponding monolingual segment of the mC4 corpus~\cite{xue2020mt5}, as \citet{ushio2023efficient}.


% \subsection{Results}

% \paragraph{Baselines}
% In Korean summarization, MuMo closely matched \textbf{AR} in quality (ROUGE-2: 20.5 vs. 20.7; ROUGE-L: 37.2 vs. 36.1) while significantly enhancing generation speed by 59\% (45.0 vs. 22.3 tokens/sec). 
% For translation, MuMo maintained a high BLEU score (20.9) and nearly doubled the speed (52.7 tokens/sec, 1.59x speed up). 
% In the MT-bench, MuMo improved the score to 5.31 and increased speed by 52\% (42.9 tokens/sec).
% Japanese benchmarks showed similar trends. MuMo's summarization scores (ROUGE-2: 13.7; ROUGE-L: 29.5) were accompanied by a 41\% speed increase (44.3 tokens/sec). 
% In translation, despite a slight decrease in BLEU score (25.8 vs. 26.3), MuMo achieved a 43\% faster generation rate (47.8 tokens/sec). 
% The MT-bench task also demonstrated a speed improvement of 68\% (42.2 tokens/sec), with a marginal score difference (4.27 vs. 4.31).
% \textbf{Spec.} baseline provided limited speed benefits and was outperformed by MuMo in both languages and across all tasks. Notably, Spec did not report generation speed for the Japanese translation task.

% \paragraph{MuMo}
% In summary, MuMo consistently delivered substantial improvements in generation speed across all evaluated tasks without compromising the quality of the generated text. These results highlight MuMo's potential to significantly accelerate text generation in multilingual contexts, particularly for non-alphabet languages such as Korean and Japanese.


% \input{Sections/table/vocab_expansion}

% \section{Experiment: Comparsion with Language Adaptation}
% In the section, our investigation delves into the effectiveness of monolingual vocabulary augmentation in pre-trained multilingual models. 
% Building on previous research~\cite{chau2020parsing, cui2023efficient} that has shown improvements in model performance through language-specific vocabulary enhancements and language adaptive pre-training (LAPT), we compare three variants of the Llama model:

% \subsection{Baselines}
% \noindent\textbf{Llama} utilizes the original pre-trained vocabulary and is fine-tuned on a monolingual instruction dataset.

% \noindent\textbf{\textsc{Va}}: An enhanced version of the baseline, Llama+ incorporates an augmented monolingual vocabulary, yet, like Llama, is also fine-tuned on an instruction dataset.

% \noindent\textbf{\textsc{Va}+\textsc{Lapt}}: Representing a more intensive adaptation, Llama++ not only includes the extended monolingual vocabulary \textbf{(VA)} but also undergoes additional Language adaptive pre-training \textbf{(LAPT)} using a vast corpus of language-specific pretraining corpora (60B tokens).\footnote{We leverage the off-the-shelf checkpoint from https://huggingface.co/beomi/llama-2-koen-13b} 

% \subsection{Results}
% \paragraph{Baselines}
% As depicted in the Table~\ref{tab:no_additional_resources}, the results reveal that the Llama + MuMo configuration achieves competitive performance with a ROUGE-L score of 35.9 and a BLEU score of 21.1, closely trailing the Llama++ model which scores 36.3 in ROUGE-L and 19.6 in BLEU. 
% Notably, Llama + MuMo accomplishes this with only 1 hour of GPU time, compared to the 151 hours required by \textbf{\textsc{Va} + \textsc{Lapt}}. 
% \textbf{\textsc{Va}}, despite the extended vocabulary, underperforms with a ROUGE-L of 26.1 and a BLEU of 14.2, suggesting that simply expanding the vocabulary without additional pre-training is insufficient.



% \paragraph{MuMo}
% In conclusion, the Llama + MuMo model demonstrates that it is possible to achieve near-equivalent performance to the extensively pre-trained \textbf{\textsc{Va} + \textsc{Lapt}} model. 
% This finding suggests that extensive pre-training with large corpora (as in \textbf{\textsc{Va} + \textsc{Lapt}}) may not be strictly necessary.

% For the Korean language summarization task, \textbf{MuMo} model achieved a ROUGE-2 score of 21.0 and a ROUGE-L score of 45.4, compared to the "AR" model's scores of 24.7 and 44.2, respectively. 
% Notably, the "MuMo" model demonstrated a significant increase in generation speed, processing text at 45.0 tokens per second, which is a 1.55x speedup over the "Ars" model's 29.0 tokens per second.

% In the Japanese language summarization task, \textbf{MuMo} model attained a ROUGE-2 score of 13.7 and a ROUGE-L score of 29.5. Although the ROUGE-2 score is lower than the "Ars" model's score of 16.8, the ROUGE-L score is higher than the "Ars" model's 28.2. 
% The "MuMo" model's generation speed for Japanese was 44.3 tokens per second, indicating a substantial improvement in efficiency, although the exact speedup factor over the "Ars" model is not provided in the table.
% \paragraph{Summarization}
% For Korean, \textbf{MuMo} achieved a ROUGE-2 score of 21.0 and a ROUGE-L score of 45.4, which, while slightly lower in ROUGE-2, surpassed the \textbf{Ars} model's ROUGE-L score of 44.2. 
% Moreover, \textbf{MuMo} demonstrated a 1.55x speed increase, processing at 45.0 tokens per second compared to "Ars" at 29.0 tokens per second. 
% In the Japanese summarization task, \textbf{MuMo} recorded a ROUGE-2 score of 13.7 and a ROUGE-L score of 29.5, indicating a marginal decrease in ROUGE-2 but an improvement in ROUGE-L over the "Ars" model's scores of 16.8 and 28.2, respectively. 
% The model's generation speed for Japanese was 44.3 tokens per second, showcasing a notable enhancement in efficiency. 

% Overall, the results suggest that \textbf{MuMo} can accelerate text generation significantly while maintaining or even improving the output quality in terms of the ROUGE-L metric for both Korean and Japanese summarization tasks. 
% Despite a slight decrease in the ROUGE-2 score for both languages, the increase in generation speed may offer a valuable trade-off for applications requiring faster text processing without a substantial compromise in summary quality.

% \paragraph{Translation}
% Ars achieve a BLEU score of 21.2 and processed at a rate of 33.1 tokens per second, establishing the baseline performance. MuMo demonstrates a comparable BLEU score of 21.5, indicating a slight improvement in translation quality. 
% Notably, the MuMo model exhibited a significant increase in processing speed, operating at 52.7 tokens per second, which translates to a 1.59x speed-up compared to Ars.
% Ars was marked by a BLEU score of 26.3 and a processing speed of 33.4 tokens per second. 
% MuMo, while achieving a slightly lower BLEU score of 25.8, showed enhanced processing efficiency with a speed of 47.8 tokens per second. This represents a 1.43x speed-up over Ars.

% The empirical results from the translation tasks indicate that MuMo is capable of maintaining output quality while significantly speeding up the translation process. 
% This is evident from the BLEU scores, which remained close to those of the "Ars" model, despite the considerable increase in translation speed. 
% The speed-up factors of 1.59x for Korean and 1.43x for Japanese are noteworthy, as they suggest that MuMo can enhance translation efficiency without compromising the quality of the translated text.

% \paragraph{MT-Bench}


% \subsection{Automatic Evaluation with LLM-as-judge}
% \paragraph{Single}
% \paragraph{Pairwise}



% \subsection{Qualitative Results}
% \input{Sections/table/example}


==> Sections/table/addtional_lang.tex <==
% \begin{table*}[t]
% \centering

% \begin{adjustbox}{width=0.99\textwidth}
% \begin{tabular}{c|c|cccc|ccc}
% \toprule
% {}     & {}      & \multicolumn{4}{c|}{\textbf{Summarization (0-shot)}}                                                           & \multicolumn{3}{c}{\textbf{Translation (3-shot)}} 
% % &\multicolumn{3}{c}{\textbf{MT-bench (0-shot)}}                               
% \\ \hline
% {\textbf{Lang}} & {\textbf{Method}} & 
% \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{tokens/sec} & \textbf{Speed Up} & 

% \textbf{BLEU} & \textbf{tokens/sec} & \textbf{Speed Up} 

% % &  {Score} & {tokens/sec} &\multicolumn{1}{l}{Speed Up} 
% \\
% \hline
% \multirow{2}{*}{\textsc{Es}}        
% & AR                        
% & & & & & & &
% \\ 
% & MuMo
% & & & & & & &
% \\


% \hline
% \multirow{2}{*}{\textsc{Zh}}        
% & AR
% & & & & & & &
% \\ 
% & MuMo& & & & & & &

% \\
% \hline

% \multirow{2}{*}{\textsc{De}}        
% & AR
% & & & & & & &
% \\ 
% & MuMo& & & & & & &

% \\
% \hline

% \multirow{2}{*}{\textsc{Id}}        
% & AR
% & & & & & & &
% \\ 
% & MuMo& & & & & & &

% \\


% \bottomrule

% \end{tabular}
% \end{adjustbox}
% \caption{Comparative Study with LLM Inference Baselines.
% The column labeled \textbf{Speed Up} denotes the relative performance on Auto-Regressive (AR).
% The \textbf{Boldface} highlights the optimal performances, and the second highest score is underscored.}
% \end{table*}


==> Sections/table/preprocess_algorithm.tex <==

% \begin{algorithm*}
% \caption{\jm{TODO: Preprocess Algorithm}}
%   \textbf{Document}: $\mathcal{D}_{i}= (x_0, ...,x_l) ;

%   \textbf{Target Language Vocabulary}: $\mathcal{V}_{\text{mono}}= (v_0, ... ,v_1) ;

%   \textbf{Preprocess}: ;


%   \For{$i\leftarrow 1$ \KwTo $N$}{
%         cursor=0\\
%         PhraseCollection=$\{\}$\\
%         \WHILE{cursor$\leq ||d_i||_t$}{
%             \eIf{$L_{min}$ $\leq$ len(cache$_p$) $\leq$ $L_{max}$}{
%                 label$_{now}$, rest=SearchPhrase(cache$_p$)\\
%             }{
%                 \If{len(cache$_p$) $>$ $L_{max}$}{
%                     cache$_{p}$=$\{\}$\\
%                 }
%             } 
%             \eIf{label$_{last}$ is True and label$_{now}$ is False}{
%                 cursor -= 1\\
%                 PhraseCollection.append(cache$_p$, rest)\\
%                 cache$_p$=$\{\}$
%             }{
%                \If{label$_{last}$ is False and label$_{now}$ is False}{
%                     PhraseCollection.append( cache$_p$, None)\\
%                     cache$_p$=$\{\}$
%                 }
%             }
%             cursor += 1\\
%             label$_{now}$=label$_{last}$
%         }
%         $\mathcal{D}'$.append(${\rm PhraseCollection}$)
% }
% \label{alg:preprocess}
% \end{algorithm*}

==> Sections/table/pretraining_corpus.tex <==

\begin{table}[t]
\small
\centering
\begin{adjustbox}{width=0.47\textwidth}
\begin{tabular}{lr|lr}
\toprule
Language & \multicolumn{1}{l}{Percent} & Language & \multicolumn{1}{l}{Percent} \\
\midrule
en       & 89.70\%                     & uk       & 0.07\%                      \\
unknown  & 8.38\%                      & ko       & 0.06\%                      \\
de       & 0.17\%                      & ca       & 0.04\%                      \\
fr       & 0.16\%                      & sr       & 0.04\%                      \\
sv       & 0.15\%                      & id       & 0.03\%                      \\
zh       & 0.13\%                      & cs       & 0.03\%                      \\
es       & 0.13\%                      & fi       & 0.03\%                      \\
ru       & 0.13\%                      & hu       & 0.03\%                      \\
nl       & 0.12\%                      & no       & 0.03\%                      \\
it       & 0.11\%                      & ro       & 0.03\%                      \\
ja       & 0.10\%                      & bg       & 0.02\%                      \\
pl       & 0.09\%                      & da       & 0.02\%                      \\
pt       & 0.09\%                      & sl       & 0.01\%                      \\
vi       & 0.08\%                      & hr       & 0.01\%   \\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{\textbf{Language distribution in pretraining data with percentage >= 0.005\%}. 
Most data is in English, meaning that  will perform best for English-language use cases. The large \texttt{unknown} category is partially made up of programming code data.}
\label{tab:lid}
\end{table}


% \begin{table}[t]
% \centering
% \begin{tabular}{lr|lr}
% \toprule
% Language & \multicolumn{1}{l}{Percent} & Language & \multicolumn{1}{l}{Percent} \\
% \midrule
% en       & 89.70\%                     & uk       & 0.07\%                      \\
% unknown  & 8.38\%                      & ko       & 0.06\%                      \\
% de       & 0.17\%                      & ca       & 0.04\%                      \\
% fr       & 0.16\%                      & sr       & 0.04\%                      \\
% sv       & 0.15\%                      & id       & 0.03\%                      \\
% zh       & 0.13\%                      & cs       & 0.03\%                      \\
% es       & 0.13\%                      & fi       & 0.03\%                      \\
% ru       & 0.13\%                      & hu       & 0.03\%                      \\
% nl       & 0.12\%                      & no       & 0.03\%                      \\
% it       & 0.11\%                      & ro       & 0.03\%                      \\
% ja       & 0.10\%                      & bg       & 0.02\%                      \\
% pl       & 0.09\%                      & da       & 0.02\%                      \\
% pt       & 0.09\%                      & sl       & 0.01\%                      \\
% vi       & 0.08\%                      & hr       & 0.01\%   \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Language distribution in pretraining data with percentage \textgreater{}= 0.005\%}. Most data is in English, meaning that \cinnamon{} will perform best for English-language use cases. The large \texttt{unknown} category is partially made up of programming code data.
% }
% \label{tab:lid}
% \end{table}
